Optimal Pricing for Data-Augmented AutoML Marketplaces

Organizations often lack sufficient data to effectively train machine learning (ML) models, while others possess valuable data that remains underutilized. Data markets promise to unlock substantial value by matching data suppliers with demand from ML consumers. However, market design involves addressing intricate challenges, including data pricing, fairness, robustness, and strategic behavior. In this paper, we propose a pragmatic data-augmented AutoML market that seamlessly integrates with existing cloud-based AutoML platforms such as Google's Vertex AI and Amazon's SageMaker. Unlike standard AutoML solutions, our design automatically augments buyer-submitted training data with valuable external datasets, pricing the resulting models based on their measurable performance improvements rather than computational costs as the status quo. Our key innovation is a pricing mechanism grounded in the instrumental value - the marginal model quality improvement - of externally sourced data. This approach bypasses direct dataset pricing complexities, mitigates strategic buyer behavior, and accommodates diverse buyer valuations through menu-based options. By integrating automated data and model discovery, our solution not only enhances ML outcomes but also establishes an economically sustainable framework for monetizing external data.

==> sections/economic-backup.tex <==
\section{Economic Component: Data Market Design}

\hf{We divide the assumptions to physical or mechanism-considerable. }

\subsection{Buyer Pricing}


The data pricing problem can be mathematically cast as follows, where we focus on the key economic properties of the market. 

% The data pricing problem can be mathematically cast as follows, in addition to the description previously. Please see the later section on Pricing Protocols for more information. 

\textbf{Modeling of the Buyer. } The buyer has a labelled dataset $D = \{X, Y\}$ that they wish to train the model on, as well as a unlabeled dataset $X'$ which they wish to conduct inferences and predictions on. The buyer wants inferences with labels $Y'$ associated with the dataset $X'$.  Each data buyer is captured by a private type $\theta \in \Theta$ that the buyer knows but the market does not know. We assume that there is an estimated distribution $\mu$ over buyer type $\theta$. This type characterizes the utility that the buyer receives from getting inferences. In particular, the buyer is assumed to have an (average) value function $v( q,\theta)$ for each single data point in $X'$, where $q$ is the accuracy of the trained model.\footnote{We will discuss about how to estimate $q$ later but roughly we agree that it should be based on a randomly sampled subset of the the labelled data $D$. This is further discussed in section 1.4} Thus the buyer's total value for inference is $v(q,\theta) |X'|$. Note that the total number of to-be-inferenced data points $|X'|$  is assumed to be known (since buyer needs to submit $X'$  to the platform anyway). Typically, the estimated value function $v(q:\theta)$ is assumed to be concave and non-linear. \\





% We consider the data pricing problem between the platform and a data buyer. Each data buyer is captured by a type $\theta$, associated with which is  a  (typically non-linear and concave) value function $v(q;\theta)$ that describes this buyer type $\theta$'s value for a solution quality $q \in [0,1]$.\footnote{this normalization is without loss of generality. We can also interpret $q$ as the ML algorithm's precision. }  



% The mechanism will charge the buyer for two services: (1) the service of performing the data discovery; (2) after discovering the data, the sales of the data. The first charge is primarily to compensate the platform's computation cost. The second charge is to capture the value of the data and compensate the sellers. 


% \jon{It might be the case that $X'$ is not known at the time of training but at some future point in time (for example, for predictions)} 

% \raul{$|X'|$ must be know before training, or otherwise we cannot apply vertical augmentations}

\textbf{The Interaction Protocol. } The interaction between the seller and buyer is in continuous time domain, with $t \in [0,T]$, where $T$ is the terminal time. The buyer needs to pay for the following two services during the protocol:
\begin{enumerate}
    \item The computation cost, with cost $c(t)$ per unit of time. This primarily compensates the platform for computation costs. 
    \item The data, or more precisely, the trained new inference API, which is developed based on the platform's data and possible stronger machine learning models. The performance of this API  is summarized into a quality/accuracy parameter $q$, which is the only thing that matters to the buyer's value.\footnote{More generally, the value function may depend on time $t$ or even does not depend on $|X'|$ linearly, but we do not consider that at this point. } This captures the value of the data and machine learning model and compensates the data sellers and the platform.
\end{enumerate}



% \subsubsection{Revenue-Maximizing Mechanisms for Selling Discovered Data}


% \hf{For this one, I think we can employ a real-time charge (like the charge in gas stations) which charges the buyer  $ct$ for search (data discover) time $t$, where $c$ is our true computation cost per unit of time. During this process,  the current best accuracy $q(t)$ as well as the number of total searched data sets are shown in real time to the buyer. This part does not have much mechanism design --- we just charge exactly the computation cost we suffered and the buyer can stop at any time $t$ as she wants.}

% There are four different business models that we considered. After lengthy discussion, we decided to go with model 4, which is shown below. The rest of the models are discussed in the appendix. 



\subsubsection{Treating selling data as an inference service}

Data is unlike traditional goods in that data is non-rivalrous and non-excludable, rendering traditional methods of selling data obsolete. For example, due to the non-excludable nature of data, if the buyer obtains the data directly, they can turn around and distribute it to other buyers, hence creating a massive problems. Thus, instead of selling data directly as a good, we propose to sell data as a service instead. \\

In the business model we consider, the buyer tells the market his task. We will build a model --- with possibly the help from data and model sellers --- which will be used as an API. The buyer then pays for every access to this API. We chose this business model because it focuses on essential service that the buyer wants -- conducting better inferences and predictions. This business model is both accessible to use for the buyer, and also less prone to attacks since the buyer does not have access to the underlying model. It abstracts away all the technical details of the inference and prediction service, and the buyer just needs to know how to input the dependent and independent variables as data, which allows us to cater to a wider, less tech-savy market segment. 

% Note that this differs from Model 3 since 3 sells the entire API whereas here we sell each access to the API. 

\hf{I think this may be problematic since the buyer may ask us to build a model but only access it a few times. Since ML tasks are usually very user-specific, this model may not be that useful to the users.  Then we really wasted our effort to build a model, after which the buyer does not really use it that much. }\\
    \sg{why not ask the user to pay for model training and inference (as a service) both.}\\
    
    \jon{I like this fully integrated model best, where we offer end to end services. The difference between this and 3 that I see is that 3 is a product pricing model while 4 is a subscription pricing model. From a user experience standpoint, I am a big fan of the Apple-Jobsian fully integrated user experience, where we make the experience as simple and elegant as possible to the user and black box everything else. This will make our product accessible to users who are not knowledgeable in ML -- they just need to submit their task and we run all the computations and details for them, including running their model on our servers. This is like the service models that Raul mentioned last meeting, which I really like. \\
    
    Let's think about the essence of the market: in this case, what the buyer wants fundamentally is to be able to make predictions or inferences on unseen data. In the case of predictions, they would most likely be time series tasks, with the buyer wanting to make predictions for future dates. Hence, they will need to access the interface each time they want to make a prediction in the future (imagine a stock trader trying to predict stock prices). Furthermore, they will also need \emph{future} data that we augmented their model with to make future predictions. Thus I think think they have good reason to want to access either the data or inference API continuously.\\
    
    Moreover, like we discussed in the meeting, models 3 and 4 reduce the incentive for attacks where they intentionally make their data/model noisy. Because the buyer has no access to their model and any inferences must go through the API, there is less flexibility for them to add and decrease noise.\\
    
    I think there is a middle ground between models 3 and 4 where we charge the buyer initially for model building then charge them for a subscription (possibly subsidized) like what Sainyam said. The subscription will cover computation costs of running their model and access to future data.
    }


 
\subsubsection{Jukebox Pricing Protocol}

% \jon{In our discussion, we came to the conclusion that it is not so easy to measure $q$, so I am going redefine the problem mathematically here so that the problem and language we use are consistent and introduce the evaluation problem below}

Given the discussion above, we propose the following interaction protocol, which we coin the jukebox model. 

The platform is designed to not profit from computation and thus charge the exact computation cost, i.e., cost $c(t)$ for computation time $t$. This will be made clear to any buyer at the very beginning.\footnote{This means the cost $c$ will be cheaper than current platforms like Vertex AI since they profit from such computational cost. In the future, one can also improve protocols that only charges $\alpha$ fraction of the total cost and shift some cost to the platform. This can shift the risk of search cost to the platform, and thus encourage the buyer to search more in order to find better model accuracy (which is better for user's pricing). }   

The price for the trained API is a function of the quality, denoted as $x(q)$. This pricing function is given at the beginning, before any search starts. Note that here we intentionally removed the procedure of eliciting buyer's private type $\theta$ and then design tailored pricing scheme for each buyer. Such communication procedure is typically costly and may make the system usage complicated. 

\jon{However, note that the buyer is forced to reveal the dataset $D$ and $X'$ to the platform. Hence, the platform actually has more information about the buyer's type than nothing, and can take this into account when pricing. For example, we can also price based on the size of $X'$}

% The following is trying to capture the task  difficulty $\omega \in \Omega$ that  neither the seller nor the buyer knows about. 

\textbf{Stochastic Modeling of Quality Evolution} Different task has different difficulties (or rather, fitness to the platform's data pool), which will be reflected by how fast the quality $q$ evolves as a function of training time $t$. We assume that the evolution of quality as a function of time $t$ is a stochastic  process $Q(t)$. As a convention, we use $q(t)$ to denote the realized quality at time $t$. \hf{need to do some survey about what is a good model for this and should consult with practioneers about what we can assume about $Q(t)$.  We want to capture if the average quality $q(t)/t$ is large, then the task is easy and it is more likely to have significant quality improvement in the next hour.  }   $Q(t)$ is assumed to be public knowledge --- in practice, the platform can learn this $Q(t)$ and reveal it to the buyer as a guidance for the buyer to make decisions.   Note that if the buyer terminates at time $t$, he can pick any previously realized quality $q \leq q(t)$  that she saw and terminates with a payment $x(q) + ct$. 

\jon{I did a bit of literature review to find a monotonic stochastic process, have not found anything so far. Specifically, we need something that has geometric-like properties at both ends of the bounds and is monotonic}

$Q(t)$ should have the following properties
\begin{enumerate}
    \item $Q(t)$ should be bounded between $[0,1]$
    % \item The increments $Q(t') - q(t)$ for some $t' > t$ should be independent and by property (1) have support $[0, 1-q(t)]$
    \item $Q(t)$ should be monotonic increasing. This is not well studied in the stochastic processes literature
    \item $Q(0) = 0$
    \item We can model the difficulty of each task using some unknown latent variable $\omega$
    \item $Q(t)$ should be sample-continuous
\end{enumerate}

There are two ways in which we can approach the fact that $Q(t)$ is monotonic -- 1. We find a monotonic stochastic process, or 2. We take the rolling supremum of a stochastic process. We take the second approach below in order to leverage literature on stochastic calculus, and because it makes more intuitive sense for the search process to be independent.\\


It is standard practice in the stochastic calculus literature to model any continuous process as a function of Brownian motion (Weiner process). Let $B_t$ be the underlying Brownian motion with $B_0 = 0$. Then we propose the following model for $Q_t$:
\[Q_t = \sup_{s \le t} X_s = \sup_{s \le t}  \frac{1}{1+e^{-\omega B_s}} =   \frac{1}{1+e^{-\omega \sup_{s \le t} B_s}}\]
The logistics function helps us satisfy property (1) and makes increases in $Q(t)$ easier at first. $\omega$ characterizes the difficulty of the task, with higher $\omega$ indicating more difficult tasks. Taking the supremum of a Weiner process is a studied problem in stochastic processes. Specifically, the reflection principle allows us to conclude interesting properties for the supremum. For example, on any fixed interval $[0,T]$, we know that the supremum is more likely to occur near the endpoints. \\

\textbf{Buyer's Decision Making. } The buyer, with private type $\theta$, starts by observing the pricing function $x(q)$ and unit computation cost $c$. At any given time $t \geq 0$, the buyer observes the current quality $q(t)$ and makes the following binary decision about stopping or not:
\begin{enumerate}
    \item Stop the search, in which case she receives utility $$ \max_{ q \leq q(t)} |X'|(v(\theta, q) - x(q))$$  
    
    \item Continue the search, in which case she receives expected future utility 

    $$  \max_{\tau \geq t} \bigg[ - c(\tau - t) +  \Ex_{q(\tau) \sim Q(\tau |   q(t))}\max_{q \leq q(\tau)} \big[ |X'|v((\theta, q) - x(q)) \big]    \bigg]  $$
    where $c(\tau - t) $ is the additional cost that the buyer needs to pay if she will continue search until time $\tau (\geq t)$. 
    
\end{enumerate}
Note that the buyer is solving a non-trivial optimal stopping problem. 
% \jon{A version in which the buyer can choose from previously discovered qualities is presented in section 1.5}

\textbf{Known $q(t)$}
Suppose that $Q(t) = q(t)$ is deterministic and known to the buyer beforehand. Then the optimal stopping time $t_\theta$ can be computed beforehand as
\[t_\theta = \arg_t\max[v(q(t), \theta) - c(t) - x(q(t))]\]
We know that we can assume WLOG that $c(t)$ is linear. We also assumed that $v$ is concave. Hence, as long as $x$ is chosen to be concave and $q$ is concave, then the optimum is unique and can be solved using standard analytical techniques. In particular, the FOC is
\[v^1(q(t), \theta)q^1(t) - k - x^1(q(t))q^1(t) = 0\]


\textbf{Platform's Mechanism Design Problem. } The platform simply picks the best pricing function $x(q)$ to maximize revenue, with knowledge on all other game parameters, including the distribution $f(\theta)$ of buyer's type $\theta$.  


% We provide inferences/predictions of different qualities $q$. Let $Y_q$ denote the predictions made by a model with quality $q$. Then we will assume that $\tilde{v}(\theta, Y_{q'}) \le \tilde{v}(\theta, Y_q)$ for all $q' \le q$. We elaborate more on how to evaluate $q$ below. Statistically, we can model $q$ as a latent variable.\\

\jon{There are some assumptions we need to clarify on the data market side. Specifically, how is search conducted, and what assumptions we can make regarding computation costs. I coarsely generalized the search space here.}

There cost for the market to search and train a model on augmented data is captured by a cost function $c(q, \omega)$. Specifically, the computation cost depends on the task difficulty $\omega$. Note that we are assuming that we also train the model while we are searching.\\

Future inferences using the model incur further costs $c(n, \omega, q)$, where $n$ is the number of inferences that we make. 

We shall make the following assumptions:

\begin{enumerate}
    \item Computation resources are easily scalable. Thus, computation costs for each buyer only depends on $q$ and $\omega$, and does not depend on how many other buyers there are in the market. Optimal computation scheduling is another interesting but perhaps separate question. 
    \item There exists some quality measure $q: Y \rightarrow [0,1]$ such that $\tilde{v}(\theta, Y') \le \tilde{v}(\theta, Y)$ for all predictions $Y', Y$ such that $q(Y') \le q(Y)$. Thus, $v(q,\theta)$ is monotonically increasing in $q$ for any $\theta$. 
    \item There is not minimum cost that we need to pay the sellers. It is free to share data, so these costs do not need to be considered
    \item Both $X$ and $X'$ are i.i.d. generated from some population distribution $(X, Y), (X', Y') \sim Pop$. This ensures PAC-learning guarantees
\end{enumerate}

% Let $F$ be the class of models we are considering, parameterized by parameters $\phi \in \Phi$. Specifically, $f_\phi: X \rightarrow Y$ takes as input $X$




 
 \subsubsection{Model Accuracy Evaluation}
 
 We need to figure out how to access the quality $q$ of the model in order to charge the buyer the right amount (if we are charging by $q$ instead of cost). Presumably this requires us to test the model on a validation set. We will call the labeled data set $D = \{X,Y\}$ and the unlabeled dataset that the buyer wants to conduct inferences on $X'$. There are three ways we can do this:
 
\begin{enumerate}
    \item The buyer chooses the validation set $D_v \subset D$, which is hidden from the market. The market only gets to see $D-D_v$. The problem with this is that the buyer can game the system by choosing a very difficult validation set so that our validation accuracy is low. Moreover, it is difficult to implement the jukebox pricing protocol if the buyer is in charge of validation
    \item The buyer reveals $D$ to the market and the market chooses the validation method. The problem with this is that the market needs to convince the buyer that the validated accuracy is correct \raul{we can solve this challenge with the escrow}. We also need to choose a validation strategy that robust \raul{this is an interesting challenge: how to price the 'error'}. In particular, cross validation might be a good validation benchmark. The buyer could also try to game this benchmark by introducing noise into the $D$, for example, by adding irrelevant data points. It is unclear at the moment whether the buyer is incentivized to conduct such an adversarial attack, since adding noise would potentially decrease the model accuracy on $X'$. We need to answer the follow questions with regards to this method:
    \begin{enumerate}
        \item How do we avoid strategic attacks?
        \item How do we ensure coverage on all of $D$? Should we aim for coverage on all of $D$? Should we augment the data differently and use separate models? Coverage is very important since we want to make sure that we can produce inferences on $X'$. \jon{I am personally of the opinion that we can just use NA for data that is missing and create an ensemble model that covers all of $D$. }
    \end{enumerate}
    \item We estimate $q$ using some other method that does not involve validating the model on data. For example, this could involve some prior over the tasks, and we could estimate $q$ based on the difficulty of the task. The problem with this is that it is unclear how accurate our estimate is going to be. Validating on the data is still our best guess at $q$. Note that any evaluation method that uses information from this buyer is potentially open to attacks. 
    \jon{Raul is strongly against priors, and I think I would agree that measurement seems difficult, though this seems like a problem best answered in practice}
\end{enumerate}

Note that these three methods are not exclusive -- we can use some combination of them in the end.

\subsection{Revenue Allocation}

TBD

\subsection{Optimal Pricing through Numerical Optimization}

Assume that $q$ is discrete, $t$ is discrete, and $\theta$ is discrete. Furthermore, assume that $q(t)$ is deterministic. Then there is no difference between choosing a $q$ and choosing a $t$. Let $u(q, \theta)= v(q, \theta) - c(q)$, the utility that the buyer of type $\theta$ gets for choosing $q$ without pricing. Then we can then calculate the optimal pricing policy numerically as follows:

\begin{enumerate}
    \item Initialize a vector of optimal $\boldsymbol{q}_\theta$
    \item Initialize a vector of the pricing policy $\boldsymbol{x}_q$
    \item Set the optimand as $\sum_\theta \mu(\theta) x(q(\theta))$
    \item Set constraints $u(q_\theta, \theta) - x(q_\theta) \ge u(q, \theta) - x(q) \quad \forall q, q_\theta$
    \item Solve using optimizer of choice
\end{enumerate}

==> sections/openproblem.tex <==
\section{Open Questions}

% \begin{itemize}
%     \item How do we avoid the attack in which the buyer extracts the underlying dataset and resells that data through their model?
%     \item How do we avoid an attack in which the buyer introduces noise?
%     \item Who owns the inferences generated by the model? Currently we are assuming that the buyer does, but the inferences are based on data from the sellers, so it might be fair to give the sellers some amount of ownership over the new data?
%     \item If we discover two data augmentations that achieve the same $q$, which augmentation do we use?
%     \item How do we optimize both data search and model search?
% \end{itemize}

% \subsection{Notes from Oct 27 Meeting}
% \begin{itemize}
%     \item Buyers might manipulate the scoring/accuracy/quality function in order to be charged less
%     \item It is hard to predict the value of a dataset (cannot do market research, etc.)
%     \item Can try to run credible mechanism
%     \item How do we deal with a prior?
%     \item What if we discover a cheaper solution later on?
%     \item We are providing a derived data product?
%     \item We need to incentivize sellers to sell data to the market
%     \item Can we require that the buyer submit their data too?
% \end{itemize}

% \subsection{Other Notes}

% Conferences we are interested in: ICML, WWW, EC, SIGMOD/VLDB


==> sections/system.tex <==
\section{Discovery Engine: Efficient Data and Model Discovery}
\label{sec:system}
% \hf{maybe try our best to shorten this to 1 page -- most important thing is to discuss what the reader should be surprised about, or what novelty we are most pround of. Other small details can be described in high-level and defer details to Appendix. Based on discussions: the most important insight seems to be that we need to train only one model for each round which reduces model training from $log P \times M$ to $log P + M$. This is indeed interesting, but why? May need Sainyam to explain. In particular, it is not clear to me why the following sentence in the proof of Prop 1 is correct/valid "Further, the sequential querying strategy chooses the best augmentation in each iteration (this holds for any model because the best augmentation according to $M^*$ is also the best according to any other model $M$)."     }




% \hf{I moved the following definitions from earlier version of Sec 3 to here, though I feel these can all be   deleted  as I think they do not seem to be really needed? I stil put them here just in case. 

% \begin{definition}[Data Collection]
% A  data collection contains a set of datasets $\mathcal{D}= \{D_1,\ldots, D_n\}$, where different datasets $D_i,D_j$ may contain overlapping values. In this work, we assume each dataset $D_i$ is tabular, as is common in many enterprise scenarios.
% \end{definition}

% \begin{definition}[Join Path]
% A join path $P$ is defined as an ordered list of datasets $P\equiv \{D_1,\ldots, D_t\}$ such that datasets $D_j$ and $D_{j+1}$ join for all $j<t$ with each other forming a chain of join operations. We say the original dataset $\din$ can be augmented using $t$ datasets.
% % The dataset formed by joining these $t$ datasets is considered to be augmented with the original dataset $\din$.
% \end{definition}

% Adding additional features using such database joins and searching across different ML models could help to improve the performance metric of a model. Thus, identifying profitable join paths is one way of doing feature engineering.

% \begin{problem}[Data and Model (DnM) Discovery]
% \label{prob:discovery}
% Given a training dataset $D_{tr}$, a set of join paths $\mathbf{P}$ (where each join path translates to a different augmentation), a collection of ML models $\mathbf{M}$, identify a minimum set of augmentations $T\subseteq \mathbf{P}$ and an ML model $M\in \mathbf{M}$ such that $m(M\leftarrow (D_{tr}\Join T))$ is maximized. 
% \end{problem}
 

% \mypar{Data Collection} A collection of datasets, $\mathcal{D}= \{D_1,\ldots, D_n\}$, that are used by the market to discover augmentations by joining with the initial data $D_{tr}$. 
% In this paper, we assume the platform fully owns these datasets, e.g., a large company seeking to monetize access to their data. In a more general setting, these datasets could come from different owners.



%\notera{more justification}


% \mypar{\textcircled{\raisebox{-0.9pt}{2}} Search} The \textit{discovery engine} takes the buyer's task and searches for data augmentations, $D = (D_{tr}, D_{val}, D_{te})$ using the discovery index. The discovery engine incrementally produces a list of ($D_i$, $q_i$) pairs, where $D_i$ denotes an augmentation, and $q_i$ denotes the associated metric value computed using this augmentation, on the test data or cross-validation. We build upon current discovery techniques \cite{galhotra2023metam} to implement  discovery engine.

% }

Recall that our pricing mechanism requires a sequence of model performance metrics to create the menu of metric-price pairs. We now study how to effectively discover data augmentations and ML models to produce the sequence of metrics for the user's downstream task.

A trivial approach to the data and model discovery problem is to consider every combination of sets of augmentations $\mathbf{P}$ and ML models $\mathbf{M}$. This approach gives the optimal solution, but it is intractable to train $O(2^{|\mathbf{P}|} |\mathbf{M}|)$ models where $|\mathbf{P}|$ is often in the order of millions. Longer runtime translates into higher search costs that reduce the number of buyers who benefit from the market. Prior data discovery methods have studied ways to prune the search space in settings where the downstream model is fixed. Specifically, Metam~\cite{galhotra2023metam} leverages properties of the data (datasets that are similar often yield similar performance metrics on ML models) to prune irrelevant augmentations and prioritizes them in the order of their likelihood to benefit the end user.

A direct adaption of the technique from \cite{galhotra2023metam} would rank the different augmentations and trains an ML model to test the top-ranked augmentation, then use the performance of the trained model as feedback to re-rank other augmentations iteratively. This approach has been shown to converge in $O(\log{\mathbf{P}})$ rounds of testing the top-ranked augmentation, requiring us to train a new model whenever the top-candidate augmentation is tested, leading to $O( |\mathbf{M}| \times \log |\mathbf{P}|)$ model trainings in total. While theoretically feasible, it is time-consuming and expensive to train thousands of models. 

In this work, we present an efficient mechanism to choose the best dataset and model simultaneously. Specifically, we model each ML model as an arm and simulate a bandit-based learning problem to choose the best model. Note that our problem is similar to pure exploration framework, as the goal is to choose the best model and stop exploration after that\footnote{Even though the goal is to stop after choosing the best arm, the best arm is relative to the input datasets which evolves over time. We model this variation as an adversarial bandit. Theoretically analyzing the effect of the evolution of the ML model is an interesting question for future work.}.

\begin{algorithm}[tbh]
\small
    \caption{\textsc{Model Discovery Algorithm}}
    \label{alg:discovery}
     \textbf{Input}: Training Data $D_{tr}, D_{val}$, List of Models $\mathbf{M}$, Augmentations $\mathbf{P}$\\
     \noindent \textbf{Output}: ML Model $M$ \quad \quad \quad\quad\quad\,
    \begin{algorithmic}[1] %[1] enables line numbers
        \STATE Initialize the solution set of augmentations $\mathbf{T}\leftarrow \phi$ \\
        \STATE Initialize $w(M) = 1,  \forall M\in \mathbf{M}$, $\gamma=0.1$
        \WHILE{$i\leq \textsc{StoppingCriterion}$} 
        \STATE Choose a candidate augmentation $T_i\subseteq \mathbf{P}$
        \STATE Set $\texttt{Pr}(M) =  (1-\gamma ) \frac{w(M)}{\sum_{M\in \mathbf{M}} w(M)} + \frac{\gamma}{|\mathbf{M}|}$
        \STATE $M_i\leftarrow $Sample a model $M$ according to the  probability distribution $\texttt{Pr}$.
        \STATE Update $w(M_i) = w(M_i) e^{\gamma \hat{r}(M)}/|\mathbf{M}|$, where $\hat{r}(M) = m(M_i\leftarrow (D_{in}\Join T_i))*1.0/Pr(M_i)$
        \STATE $u(T_i)\leftarrow m(M_i\leftarrow (D_{in}\Join T_i))$
        \ENDWHILE
    \STATE $\hat{T}\leftarrow \arg \max \{u(T), ~ \forall T\in \mathbf{P}\}$
    \STATE \textsc{Return} $arg \max_{M} m(M\leftarrow D_{in},\hat{T})$
    \end{algorithmic}
    \end{algorithm}


Algorithm~\ref{alg:discovery} presents the pseudocode of our proposed mechanism. It uses Exp3 (Exponential-weight algorithm for Exploration and Exploitation, \cite{auer2002nonstochastic}) to choose the best arm.
We initialize each model with an equal weight of $1$. In each iteration, we estimate the probability of choosing a model as 
$\texttt{Pr}(M) =  (1-\gamma ) \frac{w(M)}{\sum_{M\in \mathbf{M}} w(M)} + \frac{\gamma}{|\mathbf{M}|}$, where $\gamma$ is the exploration parameter. 
% Setting $\gamma = 1$ is equivalent to choosing a random model each time.
A model is chosen based on this probability distribution and trained on the initial dataset augmented with augmentation $T_i$. The augmentation $T_i$ is chosen according to a sampling based approach from~\cite{galhotra2023metam}. This approach clusters the augmentations in $\mathbf{P}$ and greedily chooses the best augmentation by diversifying the search process across clusters. This greedy algorithm iteratively picks the best augmentation which achieves the maximum marginal gain in the metric. The metric $m$ evaluated on the trained model is used as the reward to update $w(M)$. The main advantages of the Exp3 algorithm are that the adversarial bandit-based formulation helps to model the changing input dataset in each iteration and it has shown superior empirical performance in practical scenarios~\cite{bubeck2009pure}. The \textsc{StoppingCriterion} implements the \emph{anytime} property, letting buyers stop searching whenever they want.
Algorithm~\ref{alg:discovery} trains a single ML model in each iteration as opposed to $|\mathbf{M}|$ trainings by prior techniques. We present the following result about the effectiveness of our algorithm, when it can identify a constant approximation of the optimal solution by training  $O(\log |\mathbf{P}|)$ ML models.

\begin{proposition}
    Given an initial dataset $D_{in}$, set of augmentations $\mathbf{P}$ and ML models $\mathbf{M}$, our algorithm identifies a solution $T\subseteq \mathbf{P}$ and $\hat{M}\in \mathbf{M}$ in $O(\log (|\mathbf{P}|) + |\mathbf{M}| )$ ML model trainings such that 
    $$m(\hat{M}\leftarrow D_{in}\Join T) \geq m(M^*\leftarrow D_{in}\Join T^*) \times \left(\frac{1}{\alpha}(1-e^{-\alpha \eta}) - k\epsilon \right)$$ in cases where the best augmentation for the most powerful model is no worse than other augmentations for other models. $T^*, M^*$ denote the optimal solution and
    $k,\epsilon$ are constants, $\alpha$ and $\eta$ are curvature and submodularity ratio of $m$.\label{thm:discovery}
\end{proposition}

This result indicates that the discovery approach is highly efficient in identifying useful augmentations and is capable of generating a solution at any point of time, allowing the buyer to stop whenever needed based on their measure of utility $u^{\theta}(q,x,c)$. 
% Our approach is the first to do data and model search effectively and efficiently. 
The use of the Exp3 algorithm to interleave between the model and the dataset search helps to reduce the computational complexity of the naive approach without loss in quality. We evaluated the advantages of our choice empirically in Section 5. More details on how we choose the candidate augmentation in each iteration, as well as a proof of Proposition \ref{thm:discovery}, is given in Appendix \ref{appd:discovery}.

